A simple characterization of Quillen adjunctions

We observe that an enriched right adjoint functor between model categories which preserves acyclic fibrations and fibrant objects is quite generically a right Quillen functor.

==> Contents/PackagesAndOperators.tex <==
\usepackage[english,activeacute]{babel}
\usepackage{etex}
\usepackage[latin1]{inputenc}
\usepackage[all]{xy}
\usepackage[latin1]{inputenc}
\usepackage{xypic,color}
\usepackage{latexsym}
\usepackage{mathtools}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{wasysym}
\usepackage{mathrsfs}
\usepackage{euscript}
\usepackage{amsthm}
\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{cancel}
\usepackage{graphicx,color}
\usepackage{multicol}
\usepackage{color}
\usepackage{multirow}
\usepackage{makeidx}
\usepackage{upgreek}
\usepackage{setspace} 
\usepackage{import}
\usepackage{float}
\usepackage{mleftright}
\usepackage{stmaryrd}
\usepackage{diagbox}

%BINOMIOS CON BRACKETS PARA MAPPING SPACES
\newcommand{\brbinom}[2]{\genfrac{[}{]}{0pt}{}{#1}{#2}}

%\usepackage{scalerel}
%%\setlength{\oddsidemargin}{0mm} 
%%\setlength{\hoffset}{0mm}
%\setlength{\textwidth}{200mm}
%\setlength{\oddsidemargin}{-3mm}
%\setlength{\evensidemargin}{-3mm} 
%\setlength{\textheight}{240mm}   %Estaba en 245
%%\setlength{\topmargin}{-8mm}





\usepackage{bbold}

%\usepackage[all, 2cell]{xy}
%\UseAllTwocells


\usepackage{tikz}
\usepackage{tikz-cd}
\usetikzlibrary{matrix,arrows,calc,decorations.pathmorphing,fit,shapes.geometric,decorations.pathreplacing,positioning,snakes}

%\usepackage{tikz}

\usepackage{xcolor}
\definecolor{babyblueeyes}{rgb}{0.54, 0.81, 0.94}
\definecolor{blizzardblue}{rgb}{0.67, 0.9, 0.93}
\definecolor{blue(munsell)}{rgb}{0.0, 0.5, 0.69}
\definecolor{bluegray}{rgb}{0.4, 0.6, 0.8}
\definecolor{bondiblue}{rgb}{0.0, 0.58, 0.71}
\definecolor{cadetblue}{rgb}{0.37, 0.62, 0.63}
\definecolor{carolinablue}{rgb}{0.6, 0.73, 0.89}
\definecolor{cinnamon}{rgb}{0.82, 0.41, 0.12}
\definecolor{darkcandyapplered}{rgb}{0.64, 0.0, 0.0}
\definecolor{darkcyan}{rgb}{0.0, 0.55, 0.55}
\definecolor{darkmidnightblue}{rgb}{0.0, 0.2, 0.4}
\definecolor{darkpastelblue}{rgb}{0.47, 0.62, 0.8}
\definecolor{frenchblue}{rgb}{0.0, 0.45, 0.73}

%\newcommand{\contrastcolor}{frenchblue}%{Blue3}
%\newcommand{\headingscolor}{frenchblue}
\usepackage{url}
\usepackage[bookmarksopen,colorlinks,allcolors=frenchblue,urlcolor=frenchblue]{hyperref}



\makeindex

\usepackage{scalerel}

%\usepackage[applemac]{inputenc}  % Para TeXShop

%\setlength{\oddsidemargin}{0mm} 
%\setlength{\hoffset}{0mm}
%\setlength{\textwidth}{165mm}
%\setlength{\oddsidemargin}{-2.5mm}
%\setlength{\evensidemargin}{-2.5mm} 
%\setlength{\textheight}{245mm}
%\setlength{\topmargin}{-8mm}

%\usepackage{hyperref}
\usepackage{wrapfig}
\usepackage{ifpdf}

\usepackage{syntonly}
%\includeonly{Doc_b}

\DeclareMathOperator{\ob}{\mathsf{ob}}
\DeclareMathOperator{\id}{\mathsf{id}}

\DeclareMathOperator{\hocolim}{\mathsf{hocolim}}
\DeclareMathOperator{\holim}{\mathsf{holim}}
\DeclareMathOperator{\col}{\mathsf{col}}
\DeclareMathOperator{\source}{\mathsf{s}}
\DeclareMathOperator{\target}{\mathsf{t}}

\DeclareMathOperator{\upa}{\textup{a}}
\DeclareMathOperator{\upk}{\textup{k}}
\DeclareMathOperator{\upe}{\textup{e}}
\DeclareMathOperator{\upf}{\textit{f}}
\DeclareMathOperator{\upg}{\textit{g}}
\DeclareMathOperator{\uph}{\textit{h}}
\DeclareMathOperator{\upi}{\textit{i}}
\DeclareMathOperator{\upj}{\textit{j}}
\DeclareMathOperator{\upn}{\textup{n}}
\DeclareMathOperator{\upm}{\textup{m}}
\DeclareMathOperator{\upr}{\textup{r}}
\DeclareMathOperator{\upb}{\textup{b}}
\DeclareMathOperator{\upo}{\textup{o}}
\DeclareMathOperator{\upp}{\textit{p}}
\DeclareMathOperator{\upq}{\textit{q}}
\DeclareMathOperator{\upt}{\textup{t}}
\DeclareMathOperator{\upu}{\textit{u}}
\DeclareMathOperator{\upc}{\textup{c}}
\DeclareMathOperator{\upd}{\textup{d}}
\DeclareMathOperator{\upv}{\textit{v}}

\DeclareMathOperator{\C}{\EuScript{C}}
\DeclareMathOperator{\Op}{\EuScript{O}}
\DeclareMathOperator{\E}{\EuScript{E}}
\DeclareMathOperator{\D}{\EuScript{D}}

\DeclareMathOperator{\M}{\EuScript{M}}
\DeclareMathOperator{\OpN}{\EuScript{N}}
\DeclareMathOperator{\OpB}{\EuScript{B}}
\DeclareMathOperator{\OpI}{\EuScript{I}}
\DeclareMathOperator{\OpQ}{\EuScript{Q}}
\DeclareMathOperator{\OpP}{\EuScript{P}}


\DeclareMathOperator{\V}{\EuScript{V}}
\DeclareMathOperator{\Scurl}{\EuScript{S}}

\DeclareMathOperator{\Frect}{\mathsf{F}}
\DeclareMathOperator{\Srect}{\mathsf{S}}
\DeclareMathOperator{\Grect}{\mathsf{G}}
\DeclareMathOperator{\Xrect}{\mathsf{X}}
\DeclareMathOperator{\Yrect}{\mathsf{Y}}
\DeclareMathOperator{\Zrect}{\mathsf{Z}}
\DeclareMathOperator{\Trect}{\mathsf{T}}
\DeclareMathOperator{\Nrect}{\mathsf{N}}
\DeclareMathOperator{\Mrect}{\mathsf{M}}
\DeclareMathOperator{\Qrect}{\mathsf{Q}}
\DeclareMathOperator{\Rrect}{\mathsf{R}}
\DeclareMathOperator{\Arect}{\mathsf{A}}
\DeclareMathOperator{\Brect}{\mathsf{B}}
\DeclareMathOperator{\Crect}{\mathsf{C}}
\DeclareMathOperator{\Vrect}{\mathsf{V}}
\DeclareMathOperator{\Wrect}{\mathsf{W}}
\DeclareMathOperator{\Urect}{\mathsf{U}}
\DeclareMathOperator{\Drect}{\mathsf{D}}
\DeclareMathOperator{\Orect}{\mathsf{O}}
\DeclareMathOperator{\Irect}{\mathsf{I}}
\DeclareMathOperator{\Jrect}{\mathsf{J}}
\DeclareMathOperator{\Lrect}{\mathsf{L}}
\DeclareMathOperator{\Krect}{\mathsf{K}}
\DeclareMathOperator{\Erect}{\mathsf{E}}


\DeclareMathOperator{\ACof}{\mathsf{ACof}}
\DeclareMathOperator{\AFib}{\mathsf{AFib}}
\DeclareMathOperator{\Cof}{\mathsf{Cof}}
\DeclareMathOperator{\Fib}{\mathsf{Fib}}



\DeclareMathOperator{\Rfrak}{\mathfrak{R}}
\DeclareMathOperator{\Qfrak}{\mathfrak{Q}}
\DeclareMathOperator{\Dfrak}{\mathfrak{D}}

\DeclareMathOperator{\Ho}{\mathsf{Ho}}
\DeclareMathOperator{\Fun}{\mathsf{Fun}}
\DeclareMathOperator{\Eq}{\mathsf{Eq}}
\DeclareMathOperator{\Map}{\mathsf{Map}}
\DeclareMathOperator{\HOM}{\EuScript{H}\mathsf{om}}
\DeclareMathOperator{\h}{\mathsf{h}}
\DeclareMathOperator{\Mult}{\mathsf{Mult}}
\DeclareMathOperator{\Loc}{L}


\DeclareMathOperator{\chupachup}{\scaleobj{0.6}{\multimap}}
\DeclareMathOperator{\chupachups}{\rotatebox{90}{$\chupachup$}}



\DeclareMathOperator{\Ch}{\mathsf{Ch}}

\DeclareMathOperator{\emp}{{\raisebox{.4mm}{\o}}}
\DeclareMathOperator{\pt}{\mathrm{pt}}
%\DeclareMathOperator{\lim}{lim}

\DeclareMathOperator{\colim}{colim}
\DeclareMathOperator{\Spc}{\EuScript{S}pc}
\DeclareMathOperator{\Spt}{\EuScript{S}pt}
\DeclareMathOperator{\Alg}{\mathsf{Alg}}
\DeclareMathOperator{\pFac}{\mathsf{pFac}}
\DeclareMathOperator{\Fac}{\mathsf{Fac}}

\DeclareMathOperator*{\Bigcdot}{\scalerel*{\cdot}{\bigodot}}

\newcommand{\inters}[1]{\underset{#1}{\wedge}}


\usepackage{titlesec}

%\titleformat{\chapter}[hang]
%{\vspace{-3cm}
%\normalfont\LARGE\bfseries
%}{
%\chaptertitlename\:\, 
%\thechapter}{14pt}{}
%\titleformat{\section}[hang]
%{\vspace{0pt}
%\normalfont\Large\bfseries
%}{
%\chaptertitlename\:\, 
%\thesection}{14pt}{}
%\titleformat{\subsection}[hang]
%{\vspace{0pt}
%\normalfont\large\bfseries
%}{
%\chaptertitlename\:\, 
%\thesubsection}{14pt}{}


%\titleformat{\chapter}[hang]{\scshape}{}{0pt}
%\titleformat{\section}[block]{\scshape}{}{0pt}%{hbefore-codei}[hafter-codei]



\usepackage{float}

\usepackage{fancyhdr}
\pagestyle{fancy}
%\renewcommand{\chaptermark}[1]{\markboth{#1}{}} 
%\renewcommand{\sectionmark}[1]{\markright{\thesection\ #1}}\fancyfoot[C]{\slshape \thepage}
% encabezados
%\lhead[\textcolor{frenchblue}{\thepage}]{\rightmark}
%\chead[]{}
%\rhead[\leftmark]{\textcolor{frenchblue}{\thepage}}
%\renewcommand{\headrulewidth}{0.5pt}

%\fancyhf{}
%\fancyhead[RE]{\nouppercase{\slshape\leftmark}}
%\fancyhead[LO]{\nouppercase{\slshape\rightmark}}
%\fancyhead[LE,RO]{\bfseries\thepage}


% pie y alto de pagina
\lhead[]{}
\chead[]{}
\rhead[]{}
\renewcommand{\headrulewidth}{0pt}
%\lfoot[]{}
%\cfoot[]{}
%\rfoot[]{}
%\renewcommand{\footrulewidth}{0pt}

% primera pagina de un capitulo
%\fancypagestyle{plain}{
%	\fancyhead[L]{}
%	\fancyhead[C]{}
%	\fancyhead[R]{}
%	\fancyfoot[L]{}
%	\fancyfoot[C]{}
%	\fancyfoot[R]{}
%	\renewcommand{\headrulewidth}{0pt}
%	\renewcommand{\footrulewidth}{0pt}
%}





\renewcommand{\thefootnote}{\roman{footnote}}



%FLECHA DE FUNCTOR GENERALIZADA


\usepackage{tikz}
\usetikzlibrary{calc,decorations.pathmorphing,shapes}

\newcounter{sarrow}
\newcommand\xrsquigarrow[1]{%
\stepcounter{sarrow}%
\mathrel{\begin{tikzpicture}[baseline= {( $ (current bounding box.south) + (0,-0.5ex) $ )}]
\node[inner sep=.5ex] (\thesarrow) {$\scriptstyle #1$};
\path[draw,<-,decorate,
  decoration={zigzag,amplitude=0.7pt,segment length=1.2mm,pre=lineto,pre length=4pt}] 
    (\thesarrow.south east) -- (\thesarrow.south west);
\end{tikzpicture}}%
}

